CO-Driven Activity in Comet C/2017 K2 (PANSTARRS)

Comet C/2017 K2 (PANSTARRS) was discovered by the Pan-STARRS1 (PS1) Survey on 2017 May 21 at a distance 16.09 au from the Sun, the second most distant discovery of an active comet. Pre-discovery images in the PS1 archive back to 2014 and additional deep CFHT images between 2013 May 10-13 showed the comet to be active at 23.75 au. We derive an upper limit to the nucleus radius of $R_N$=80 km, assuming a 4\% albedo. The spectral reflectivity of the comet surface is similar to "fresh" regions seen on comet 67P/Churyumov-Gerasimenko using the $Rosetta$ OSIRIS camera. Pre-discovery photometry combined with new data obtained with Megacam on the CFHT show that the activity is consistent with CO-ice sublimation and inconsistent with CO$_2$-ice sublimation. The ice sublimation models were run out to perihelion in 2022 at 1.8 au to predict the CO production rates, assuming that the outgassing area does not change. Assuming a canonical 4\% active surface area for water-ice sublimation, we present production rate ratios, $Q_{\rm CO}$/$Q_{\rm H2O}$, for a range of nucleus sizes. Comparing these results with other CO-rich comets we derive a lower limit to the nucleus radius of $\sim$14 km. We present predictions for $Q_{\rm CO}$ at a range of distances that will be useful for planning observations with JWST and large ground-based facilities.

==> Tab-Data.tex <==
\begin{longrotatetable}
\begin{deluxetable*}{lcccccccccl}
%\tabletypesize{\small}
\tablecaption{Observing Geometry and Photometry \label{tab:data}}
\tablehead{
\colhead{UTDate                    } &
\colhead{JD\tablenotemark{a}       } &
\colhead{$r$\tablenotemark{b}      } &
\colhead{$\Delta$\tablenotemark{b} } &
\colhead{$\alpha$\tablenotemark{b} } &
\colhead{TA\tablenotemark{c}       } &
\colhead{Filt                      } &
\colhead{\# Images                 } &
\colhead{mag$\pm$$\sigma$          } &
\colhead{r$_{mag}$$\pm$$\sigma$\tablenotemark{d}} &
\colhead{Color/Comment}
}
\startdata
\multicolumn{11}{l}{\bf PanSTARRS1 data}\\
2010/06/04 & 5352.10123	& 28.665 & 28.754 & 2.017 & -151.16 & i$_{p1}$ &  2 & $<$21.0$\pm$0.3   & $<$21.2$\pm$0.3  & Limiting mag \\
2012/08/07 & 6146.81325	& 25.061 & 25.146 & 2.306 & -149.01 & r$_{p1}$ &  2 & $<$21.8$\pm$0.3   & $<$21.8$\pm$0.3  & Limiting mag \\
2014/06/14 & 6821.46247 & 21.802 & 21.829 & 2.666 & -146.54 & i$_{p1}$ &  3 & $<$21.0$\pm$0.3   & $<$21.2$\pm$0.3  & Limiting mag \\ 
2014/06/13 & 6822.51886 & 21.797 & 21.824 & 2.667 & -146.54 & i$_{p1}$ &  3 & $<$20.7$\pm$0.3   & $<$20.9$\pm$0.3  & Limiting mag \\
2014/07/05 & 6844.27742 & 21.688 & 21.729 & 2.681 & -146.45 & i$_{p1}$ &  2 & $<$20.8$\pm$0.3   & $<$21.0$\pm$0.3  & Limiting mag \\ 
2014/03/20 & 6737.07683 & 22.221 & 22.202 & 2.569 & -146.88 & r$_{p1}$ &  2 &    20.67$\pm$0.30 & 20.67$\pm$0.30 & \\
2014/09/08 & 6908.76850 & 21.364 & 21.430 & 2.692 & -146.17 & i$_{p1}$ &  4 &    20.60$\pm$0.05 & 20.77$\pm$0.05 & \\
2015/05/06 & 7149.01152 & 20.138 & 20.122 & 2.871 & -145.09 & i$_{p1}$ &  4 &    20.10$\pm$0.04 & 20.28$\pm$0.04 & \\
2015/05/07 & 7150.00904 & 20.133 & 20.117 & 2.872 & -145.08 & i$_{p1}$ &  4 &    20.27$\pm$0.05 & 20.45$\pm$0.05 & \\
2016/05/27 & 7536.02124 & 18.088 & 18.052 & 3.211 & -143.07 & r$_{p1}$ &  4 &    19.53$\pm$0.04 & 19.53$\pm$0.04 & \\
2016/06/19 & 7558.88673 & 17.963 & 17.938 & 3.242 & -142.94 & i$_{p1}$ &  3 &    19.37$\pm$0.08 & 19.54$\pm$0.08 & \\
2016/06/21 & 7560.93624 & 17.952 & 17.928 & 3.245 & -142.93 & i$_{p1}$ &  2 &    19.37$\pm$0.06 & 19.54$\pm$0.06 & \\
2016/07/18 & 7587.88946 & 17.805 & 17.803 & 3.270 & -142.77 & i$_{p1}$ &  4 &    19.53$\pm$0.05 & 19.71$\pm$0.05 & \\
2017/04/10 & 7854.05173 & 16.322 & 16.280 & 3.519 & -141.06 & i$_{p1}$ &  4 &    19.19$\pm$0.07 & 19.36$\pm$0.07 & \\
2017/05/21 & 7894.91140 & 16.089 & 16.019 & 3.604 & -140.77 & w$_{p1}$ &  4 &    19.45$\pm$0.03 & 19.39$\pm$0.03 & Discovery \\
2017/06/16 & 7920.97821 & 15.940 & 15.874 & 3.651 & -140.59 & i$_{p1}$ &  4 &    18.85$\pm$0.04 & 19.02$\pm$0.04 & \\
2017/06/25 & 7929.91675 & 15.888 & 15.828 & 3.666 & -140.52 & w$_{p1}$ &  4 &    19.19$\pm$0.03 & 19.13$\pm$0.03 & \\
2017/08/06 & 7971.88255 & 15.646 & 15.638 & 3.715 & -140.21 & i$_{p1}$ &  4 &    18.94$\pm$0.05 & 19.11$\pm$0.05 & \\
2017/08/17 & 7982.77565 & 15.583 & 15.594 & 3.721 & -140.13 & w$_{p1}$ &  4 &    19.02$\pm$0.01 & 18.97$\pm$0.02 & \\
2017/08/30 & 7995.76736 & 15.508 & 15.542 & 3.725 & -140.03 & i$_{p1}$ &  4 &    18.78$\pm$0.04 & 18.96$\pm$0.04 & \\
2017/09/07 & 8003.77876 & 15.461 & 15.511 & 3.724 & -139.96 & i$_{p1}$ &  4 &    18.72$\pm$0.04 & 18.90$\pm$0.04 & \\
2017/06/16 & 7920.95557 & 15.940 & 15.874 & 3.651 & -140.59 & r$_{p1}$ &  4 &    18.96$\pm$0.06 & 19.14$\pm$0.06 & \\
2017/07/05 & 7939.88379 & 15.831 & 15.779 & 3.681 & -140.45 & r$_{p1}$ &  2 &    18.94$\pm$0.14 & 19.11$\pm$0.14 & \\
2017/07/07 & 7941.90196 & 15.819 & 15.770 & 3.684 & -140.43 & r$_{p1}$ &  4 &    19.24$\pm$0.11 & 19.41$\pm$0.11 & \\
2017/07/15 & 7949.87944 & 15.773 & 15.733 & 3.694 & -140.37 & r$_{p1}$ &  4 &    18.82$\pm$0.06 & 19.00$\pm$0.06 & \\
2017/07/17 & 7951.90526 & 15.762 & 15.724 & 3.696 & -140.36 & r$_{p1}$ &  4 &    19.15$\pm$0.20 & 19.33$\pm$0.20 & \\
\hline
\multicolumn{11}{l}{\bf CFHT Archival data from CADC} \\
2013/05/12 & 6424.61132 & 23.744 & 23.767 & 2.436 & -148.07 & u        &  7 &    23.09$\pm$0.17 & 20.76$\pm$0.23 & \\
\hline
\multicolumn{10}{l}{\bf CFHT new data} \\
2017/05/24 & 7898.05595 & 16.071 & 16.000 & 3.610 & -140.75 & w        &  1 &    19.292$\pm$0.007 & 19.237$\pm$0.007 & \\
2017/05/28 & 7901.92345 & 16.049 & 15.978 & 3.617 & -140.72 & g        &  1 &    19.673$\pm$0.015 & & \\
2017/05/28 & 7901.92345 & 16.049 & 15.978 & 3.617 & -140.72 & r        &  1 &    19.155$\pm$0.015 & 19.155$\pm$0.015 & (g-r) = 0.52$\pm$0.02 \\
2017/06/24 & 7928.97060 & 15.894 & 15.833 & 3.665 & -140.53 & g        &  1 &    19.539$\pm$0.012 & & \\
2017/06/24 & 7928.97049 & 15.894 & 15.833 & 3.665 & -140.53 & r        &  1 &    19.067$\pm$0.013 & 19.067$\pm$0.013 & (g-r) = 0.47$\pm$0.02 \\
2017/07/16 & 7950.83854 & 15.768 & 15.729 & 3.695 & -140.37 & r        & 12 &    19.081$\pm$0.004 & 19.081$\pm$0.004 & \\
2017/07/25 & 7990.80063 & 15.768 & 15.729 & 3.695 & -140.37 & g        &  1 &    19.567$\pm$0.011 & & (g-r) = 0.56$\pm$0.02 \\
2017/07/25 & 7990.80285 & 15.768 & 15.729 & 3.695 & -140.37 & r        &  1 &    19.007$\pm$0.012 & 19.007$\pm$0.012 & \\
2017/07/26 & 7991.80022 & 15.537 & 15.562 & 3.724 & -140.06 & u        &  2 &    21.260$\pm$0.054 & & (u-r) = 2.33$\pm$0.06 \\
2017/07/26 & 7991.80602 & 15.531 & 15.558 & 3.724 & -140.06 & g        &  1 &    19.513$\pm$0.013 & & (g-r) = 0.59$\pm$0.02 \\
2017/07/26 & 7991.80407 & 15.537 & 15.562 & 3.724 & -140.06 & r        &  3 &    18.927$\pm$0.008 & 18.927$\pm$0.008 & \\
2017/07/26 & 7991.80889 & 15.531 & 15.558 & 3.724 & -140.06 & i        &  2 &    18.758$\pm$0.013 & & (r-i)\hspace{0.1cm} = 0.17$\pm$0.02 \\
2017/09/14 & 8010.74649	& 15.421 & 15.483 & 3.723 & -139.91 & g	       &  4 &    19.483$\pm$0.005 & & (g-r) = 0.55$\pm$0.01 \\
2017/09/14 & 8010.74282	& 15.421 & 15.483 & 3.723 & -139.91 & r	       &  2 &    18.932$\pm$0.009 & 18.932$\pm$0.009 & \\
2017/09/14 & 8010.74230	& 15.421 & 15.483 & 3.723 & -139.91 & i	       &  6 &    18.761$\pm$0.008 & & (r-i)\hspace{0.1cm} = 0.17$\pm$0.01 \\
2017/09/14 & 8010.75793	& 15.421 & 15.483 & 3.723 & -139.91 & z	       &  4 &    18.721$\pm$0.024 & & (r-z) = 0.21$\pm$0.03 \\
2017/09/15 & 8011.72479	& 15.415 & 15.479 & 3.723 & -139.90 & u	       &  3 &    20.995$\pm$0.039 & & (u-r) = 2.12$\pm$0.04 \\
2017/09/15 & 8011.74031	& 15.415 & 15.479 & 3.723 & -139.90 & g	       &  5 &    19.413$\pm$0.004 & & (g-r) = 0.54$\pm$0.01 \\
2017/09/15 & 8011.75514	& 15.415 & 15.479 & 3.723 & -139.90 & r	       &  2 &    18.873$\pm$0.007 & 18.873$\pm$0.007 & \\
\enddata
\tablenotetext{a}{Julian Date -2450000.0}
\tablenotetext{b}{Heliocentric, geocentric distance (au) and phase angle (deg).}
\tablenotetext{c}{True anomaly (deg), position along orbit, TA at perihelion=0$^{\circ}$}
\tablenotetext{d}{Magnitude and error through 5$''$ radius aperture.}
\tablenotetext{e}{Magnitude and error converted to SDSS $r$ as described in the text}
\end{deluxetable*}
\end{longrotatetable}


==> widetab.tex <==
\begin{longrotatetable}
\begin{deluxetable}{lllrrrrrrll}
\tablecaption{Observable Characteristics of 
Galactic/Magellanic Cloud novae with X-ray observations\label{chartable}}
\tablewidth{700pt}
\tabletypesize{\scriptsize}
\tablehead{
\colhead{Name} & \colhead{V$_{max}$} & 
\colhead{Date} & \colhead{t$_2$} & 
\colhead{FWHM} & \colhead{E(B-V)} & 
\colhead{N$_H$} & \colhead{Period} & 
\colhead{D} & \colhead{Dust?} & \colhead{RN?} \\ 
\colhead{} & \colhead{(mag)} & \colhead{(JD)} & \colhead{(d)} & 
\colhead{(km s$^{-1}$)} & \colhead{(mag)} & \colhead{(cm$^{-2}$)} &
\colhead{(d)} & \colhead{(kpc)} & \colhead{} & \colhead{}
} 
\startdata
CI Aql & 8.83 (1) & 2451665.5 (1) & 32 (2) & 2300 (3) & 0.8$\pm0.2$ (4) & 1.2e+22 & 0.62 (4) & 6.25$\pm5$ (4) & N & Y \\
{\bf CSS081007} & \nodata & 2454596.5 & \nodata & \nodata & 0.146 & 1.1e+21 & 1.77 (5) & 4.45$\pm1.95$ (6) & \nodata & \nodata \\
GQ Mus & 7.2 (7) & 2445352.5 (7) & 18 (7) & 1000 (8) & 0.45 (9) & 3.8e+21  & 0.059375 (10) & 4.8$\pm1$ (9) & N (7) & \nodata \\
IM Nor & 7.84 (11) & 2452289 (2) & 50 (2) & 1150 (12) & 0.8$\pm0.2$ (4) & 8e+21 & 0.102 (13) & 4.25$\pm3.4$ (4) & N & Y \\
{\bf KT Eri} & 5.42 (14) & 2455150.17 (14) & 6.6 (14) & 3000 (15) & 0.08 (15) & 5.5e+20 & \nodata & 6.5 (15) & N & M \\
{\bf LMC 1995} & 10.7 (16) & 2449778.5 (16) & 15$\pm2$ (17) & \nodata & 0.15 (203) & 7.8e+20  & \nodata & 50 & \nodata & \nodata \\
LMC 2000 & 11.45 (18) & 2451737.5 (18) & 9$\pm2$ (19) & 1700 (20) & 0.15 (203) & 7.8e+20  & \nodata & 50 & \nodata & \nodata \\
{\bf LMC 2005} & 11.5 (21) & 2453700.5 (21) & 63 (22) & 900 (23) & 0.15 (203) & 1e+21 & \nodata & 50  & M (24) & \nodata \\
{\bf LMC 2009a} & 10.6 (25) & 2454867.5 (25) & 4$\pm1$  & 3900 (25) & 0.15 (203)  & 5.7e+20 & 1.19 (26) & 50 & N & Y \\
{\bf SMC 2005} & 10.4 (27) & 2453588.5 (27) & \nodata & 3200 (28) & \nodata & 5e+20  & \nodata & 61 & \nodata & \nodata \\
{\bf QY Mus} & 8.1 (29) & 2454739.90 (29) & 60:  & \nodata & 0.71 (30) & 4.2e+21  & \nodata & \nodata & M & \nodata \\
{\bf RS Oph} & 4.5 (31) & 2453779.44 (14) & 7.9 (14) & 3930 (31) & 0.73 (32) & 2.25e+21 & 456 (33) & 1.6$\pm0.3$ (33) & N (34) & Y \\
{\bf U Sco} & 8.05 (35) & 2455224.94 (35) & 1.2 (36) & 7600 (37) & 0.2$\pm0.1$ (4) & 1.2e+21 & 1.23056 (36) & 12$\pm2$ (4) & N & Y \\
{\bf V1047 Cen} & 8.5 (38) & 2453614.5 (39) & 6 (40) & 840 (38) & \nodata & 1.4e+22  & \nodata & \nodata & \nodata & \nodata \\
{\bf V1065 Cen} & 8.2 (41) & 2454123.5 (41) & 11 (42) & 2700 (43) & 0.5$\pm0.1$ (42) & 3.75e+21 & \nodata & 9.05$\pm2.8$ (42) & Y (42) & \nodata \\
V1187 Sco & 7.4 (44) & 2453220.5 (44) & 7: (45) & 3000 (44) & 1.56 (44) & 8.0e+21 & \nodata & 4.9$\pm0.5$ (44) & N & \nodata \\
{\bf V1188 Sco} & 8.7 (46) & 2453577.5 (46) & 7 (40) & 1730 (47) & \nodata & 5.0e+21  & \nodata & 7.5 (39) & \nodata & \nodata \\
{\bf V1213 Cen} & 8.53 (48) & 2454959.5 (48) & 11$\pm2$ (49) & 2300 (50) & 2.07 (30) & 1.0e+22 & \nodata & \nodata & \nodata & \nodata \\
{\bf V1280 Sco} & 3.79 (51) & 2454147.65 (14) & 21 (52) & 640 (53) & 0.36 (54) & 1.6e+21  & \nodata & 1.6$\pm0.4$ (54) & Y (54) & \nodata \\
{\bf V1281 Sco} & 8.8 (55) & 2454152.21 (55) & 15:& 1800 (56) & 0.7 (57) & 3.2e+21 & \nodata & \nodata & N & \nodata \\
{\bf V1309 Sco} & 7.1 (58) & 2454714.5 (58) & 23$\pm2$ (59) & 670 (60) & 1.2 (30) & 4.0e+21 & \nodata & \nodata & \nodata & \nodata \\
{\bf V1494 Aql} & 3.8 (61) & 2451515.5 (61) & 6.6$\pm0.5$ (61) & 1200 (62) & 0.6 (63) & 3.6e+21  & 0.13467 (64) & 1.6$\pm0.1$ (63) & N & \nodata \\
{\bf V1663 Aql} & 10.5 (65) & 2453531.5 (65) & 17 (66) & 1900 (67) & 2: (68) & 1.6e+22  & \nodata & 8.9$\pm3.6$ (69) & N & \nodata \\
V1974 Cyg & 4.3 (70) & 2448654.5 (70) & 17 (71) & 2000 (19) & 0.36$\pm0.04$ (71) & 2.7e+21  & 0.081263 (70) & 1.8$\pm0.1$ (72) & N & \nodata \\
{\bf V2361 Cyg} & 9.3 (73) & 2453412.5 (73) & 6 (40) & 3200 (74) & 1.2: (75) & 7.0e+21 & \nodata & \nodata & Y (40) & \nodata \\
{\bf V2362 Cyg} & 7.8 (76) & 2453831.5 (76) & 9 (77) & 1850 (78) & 0.575$\pm0.015$ (79) & 4.4e+21  & 0.06577 (80) & 7.75$\pm3$ (77) & Y (81) & \nodata \\
{\bf V2467 Cyg} & 6.7 (82) & 2454176.27 (82) & 7 (83) & 950 (82) & 1.5 (84) & 1.4e+22  & 0.159 (85) & 3.1$\pm0.5$ (86) & M (87) & \nodata \\
{\bf V2468 Cyg} & 7.4 (88) & 2454534.2 (88) & 10: & 1000 (88) & 0.77 (89) & 1.0e+22  & 0.242 (90) & \nodata & N & \nodata \\
{\bf V2491 Cyg} & 7.54 (91) & 2454567.86 (91) & 4.6 (92) & 4860 (93) & 0.43 (94) & 4.7e+21  & 0.09580: (95) & 10.5 (96) & N & M \\
V2487 Oph & 9.5 (97) & 2450979.5 (97) & 6.3 (98) & 10000 (98) & 0.38$\pm0.08$ (98) & 2.0e+21 & \nodata & 27.5$\pm3$ (99) & N (100) & Y (101) \\
{\bf V2540 Oph} & 8.5 (102) & 2452295.5 (102) & \nodata & \nodata & \nodata & 2.3e+21 & 0.284781 (103) & 5.2$\pm0.8$ (103) & N & \nodata \\
V2575 Oph & 11.1 (104) & 2453778.8 (104) & 20: & 560 (104) & 1.4 (105) & 3.3e+21 & \nodata & \nodata & N (105) & \nodata \\
{\bf V2576 Oph} & 9.2 (106) & 2453832.5 (106) & 8: & 1470 (106) & 0.25 (107) & 2.6e+21  & \nodata & \nodata & N & \nodata \\
{\bf V2615 Oph} & 8.52 (108) & 2454187.5 (108) & 26.5 (108) & 800 (109) & 0.9 (108) & 3.1e+21  & \nodata & 3.7$\pm0.2$ (108) & Y (110) & \nodata \\
{\bf V2670 Oph} & 9.9 (111) & 2454613.11 (111) & 15: & 600 (112) & 1.3: (113) & 2.9e+21  & \nodata & \nodata & N (114) & \nodata \\
{\bf V2671 Oph} & 11.1 (115) & 2454617.5 (115) & 8: & 1210 (116) & 2.0 (117) & 3.3e+21  & \nodata & \nodata & M (117) & \nodata \\
{\bf V2672 Oph} & 10.0 (118) & 2455060.02 (118) & 2.3 (119) & 8000 (118) & 1.6$\pm0.1$ (119) & 4.0e+21  & \nodata & 19$\pm2$ (119) & \nodata & M \\
V351 Pup & 6.5 (120) & 2448617.5 (120) & 16 (121) & \nodata & 0.72$\pm0.1$ (122) & 6.2e+21 & 0.1182 (123) & 2.7$\pm0.7$ (122) & N & \nodata \\
{\bf V382 Nor} & 8.9 (124) & 2453447.5 (124) & 12 (40) & 1850 (23) & \nodata & 1.7e+22 & \nodata & \nodata & \nodata & \nodata \\
V382 Vel & 2.85 (125) & 2451320.5 (125) & 4.5 (126) & 2400 (126) & 0.05: (126) & 3.4e+21  & 0.146126 (127) & 1.68$\pm0.3$ (126) & N & \nodata \\
{\bf V407 Cyg} & 6.8 (128) & 2455266.314 (128) & 5.9 (129) & 2760 (129) & 0.5$\pm0.05$ (130) & 8.8e+21 & 15595 (131) & 2.7 (131) & \nodata & Y \\
{\bf V458 Vul} & 8.24 (132) & 2454322.39 (132) & 7 (133) & 1750 (134) & 0.6 (135) & 3.6e+21 & 0.06812255 (136) & 8.5$\pm1.8$ (133) & N (135) & \nodata \\
{\bf V459 Vul} & 7.57 (137) & 2454461.5 (137) & 18 (138) & 910 (139) & 1.0 (140) & 5.5e+21  & \nodata & 3.65$\pm1.35$ (138) & Y (140) & \nodata \\
V4633 Sgr & 7.8 (141) & 2450895.5 (141) & 19$\pm3$ (142) & 1700 (143) & 0.21 (142) & 1.4e+21  & 0.125576 (144) & 8.9$\pm2.5$ (142) & N & \nodata \\
{\bf V4643 Sgr} & 8.07 (145) & 2451965.867 (145) & 4.8 (146) & 4700 (147) & 1.67 (148) & 1.4e+22 & \nodata & 3 (148) & N & \nodata \\
{\bf V4743 Sgr} & 5.0 (149) & 2452537.5 (149) & 9 (150) & 2400 (149) & 0.25 (151) & 1.2e+21 & 0.281 (152) & 3.9$\pm0.3$ (151) & N & \nodata \\
{\bf V4745 Sgr} & 7.41 (153) & 2452747.5 (153) & 8.6 (154) & 1600 (155) & 0.1 (154) & 9.0e+20  & 0.20782 (156) & 14$\pm5$ (154) & \nodata & \nodata \\
{\bf V476 Sct} & 10.3 (157) & 2453643.5 (157) & 15 (158) & \nodata & 1.9 (158) & 1.2e+22  & \nodata & 4$\pm1$ (158) & M (159) & \nodata \\
{\bf V477 Sct} & 9.8 (160) & 2453655.5 (160) & 3 (160) & 2900 (161) & 1.2: (162) & 4e+21  & \nodata & \nodata & M (163) & \nodata \\
{\bf V5114 Sgr} & 8.38 (164) & 2453081.5 (164) & 11 (165) & 2000 (23) & \nodata & 1.5e+21  & \nodata & 7.7$\pm0.7$ (165) & N (166) & \nodata \\
{\bf V5115 Sgr} & 7.7 (167) & 2453459.5 (167) & 7 (40) & 1300 (168) & 0.53 (169) & 2.3e+21  & \nodata & \nodata & N (169) & \nodata \\
{\bf V5116 Sgr} & 8.15 (170) & 2453556.91 (170) & 6.5 (171) & 970 (172) & 0.25 (173) & 1.5e+21 & 0.1238 (171) & 11$\pm3$ (173) & N (174) & \nodata \\
{\bf V5558 Sgr} & 6.53 (175) & 2454291.5 (175) & 125 (176) & 1000 (177) & 0.80 (178) & 1.6e+22  & \nodata & 1.3$\pm0.3$ (176) & N (179) & \nodata \\
{\bf V5579 Sgr} & 5.56 (180) & 2454579.62 (180) & 7: & 1500 (23) & 1.2 (181) & 3.3e+21 & \nodata & \nodata & Y (181) & \nodata \\
{\bf V5583 Sgr} & 7.43 (182) & 2455051.07 (182) & 5: & 2300 (182) & 0.39 (30) & 2.0e+21 & \nodata & 10.5 & \nodata & \nodata \\
{\bf V574 Pup} & 6.93 (183) & 2453332.22 (183) & 13 (184) & 2800 (184) & 0.5$\pm0.1$  & 6.2e+21 & \nodata & 6.5$\pm1$  & M (185) & \nodata \\
{\bf V597 Pup} & 7.0 (186) & 2454418.75 (186) & 3: & 1800 (187) & 0.3 (188) & 5.0e+21  & 0.11119 (189) & \nodata & N (188) & \nodata \\
{\bf V598 Pup} & 3.46 (14) & 2454257.79 (14) & 9$\pm1$ (190) & \nodata & 0.16 (190) & 1.4e+21 & \nodata & 2.95$\pm0.8$ (190) & \nodata & \nodata \\
{\bf V679 Car} & 7.55 (191) & 2454797.77 (191) & 20: & \nodata & \nodata & 1.3e+22  & \nodata & \nodata & \nodata & \nodata \\
{\bf V723 Cas} & 7.1 (192) & 2450069.0 (192) & 263 (2) & 600 (193) & 0.5 (194) & 2.35e+21  & 0.69 (195) & 3.86$\pm0.23$ (196) & N & \nodata \\
V838 Her & 5 (197) & 2448340.5 (197) & 2 (198) & \nodata & 0.5$\pm0.1$ (198) & 2.6e+21  & 0.2975 (199) & 3$\pm1$ (198) & Y (200) & \nodata \\
{\bf XMMSL1 J06} & 12 (201) & 2453643.5 (202) & 8$\pm2$ (202) & \nodata & 0.15 (203) & 8.7e+20 & \nodata & 50 & \nodata & \nodata \\
\enddata
\end{deluxetable}
\end{longrotatetable}

